FoundWright: A System to Help People Re-find Pages from Their Web-history

Re-finding information is an essential activity, however, it can be difficult when people struggle to express what they are looking for. Through a need-finding survey, we first seek opportunities for improving re-finding experiences, and explore one of these opportunities by implementing the FoundWright system. The system leverages recent advances in language transformer models to expand people's ability to express what they are looking for, through the interactive creation and manipulation of concepts contained within documents. We use FoundWright as a design probe to understand (1) how people create and use concepts, (2) how this expanded ability helps re-finding, and (3) how people engage and collaborate with FoundWright's machine learning support. Our probe reveals that this expanded way of expressing re-finding goals helps people with the task, by complementing traditional searching and browsing. Finally, we present insights and recommendations for future work aiming at developing systems to support re-finding.

==> tex/910-acknowledgement.tex <==
\section{Acknowledgments}


